Stochastic Heavy Ball with Polyak Step Size and Armijo Line Search: A General Convergence Analysis

Polyak step size (PS) and Armijo line search (ALS) have received increasing attention in stochastic optimization, with encouraging empirical performance and theoretical guarantees. However, their convergence theory for stochastic heavy ball (SHB) methods remains limited. In this work, we develop a unified convergence analysis for SHB equipped with PS and ALS. To this end, we introduce a modified Armijo rule that closely parallels the Polyak step size, together with a decoupling analysis that isolates the historical dependence induced by momentum. For SHB with standard PS and ALS, we establish expected convergence for strongly convex, convex, and non-convex objectives without interpolation or restrictive conditions on the momentum parameter. Under interpolation or strong growth, we further strengthen the results to almost sure rates and last-iterate convergence. Moreover, for general settings beyond interpolation, we prove almost sure convergence to the exact optimum or to stationarity for SHB with diminishing variants of PS and ALS. These results provide a more comprehensive theoretical view of Polyak step size and Armijo line search for stochastic heavy ball methods.

==> Sections/statements.tex <==
\subsection*{AI use statement}
We use generative AI tools to assist with language editing, technical review, and the development of experimental code.
%
The authors have reviewed the AI-assisted material and take full responsibility for the final content of this paper, including its proofs, technical claims, and experimental results.

\subsection*{Ethics statement}
This work primarily develops convergence theory for stochastic optimization methods, supported by numerical experiments on synthetic problems and public benchmark datasets.
%
It does not involve human-subject research or the collection of personal data.
%
We do not identify specific ethical concerns arising directly from the theoretical contributions.

\subsection*{Reproducibility statement}
The algorithmic definitions and assumptions are provided in Section~\ref{sec:background}, and the convergence results and conditions for diminishing step sizes are stated in Sections~\ref{sec:main_results} and~\ref{sec:diminishing}.
%
Complete proofs are provided in Appendix~\ref{appendix:assumptions_and_lemmas}, \ref{appendix:proof_of_theorems}, and \ref{appendix:diminishing}.
%
The numerical objectives, parameter choices, and reported statistics are described in Section~\ref{sec:numerical_theory_aligned}, with additional experimental settings provided in Appendix~\ref{appendix:numerical}.
